Empirical Determination of Convection Parameters in White Dwarfs I : Whole Earth Telescope Observations of EC14012-1446

We report on analysis of 308.3 hrs of high speed photometry targeting the pulsating DA white dwarf EC14012-1446. The data were acquired with the Whole Earth Telescope (WET) during the 2008 international observing run XCOV26. The Fourier transform of the light curve contains 19 independent frequencies and numerous combination frequencies. The dominant peaks are 1633.907, 1887.404, and 2504.897 microHz. Our analysis of the combination amplitudes reveals that the parent frequencies are consistent with modes of spherical degree l=1. The combination amplitudes also provide m identifications for the largest amplitude parent frequencies. Our seismology analysis, which includes 2004--2007 archival data, confirms these identifications, provides constraints on additional frequencies, and finds an average period spacing of 41 s. Building on this foundation, we present nonlinear fits to high signal-to-noise light curves from the SOAR 4.1m, McDonald 2.1m, and KPNO 2m telescopes. The fits indicate a time-averaged convective response timescale of 99.4 +/- 17 s, a temperature exponent 85 +/- 6.2 and an inclination angle of 32.9 +/- 3.2 degrees. We present our current empirical map of the convective response timescale across the DA instability strip.

==> provencaltab1.tex <==
\begin{deluxetable}{rrrcr} 
\tablecolumns{5}
\tablewidth{0pc}
%\tabletypesize{\scriptsize}
\tabletypesize{\small}
%\rotate
\tablecaption{Journal of XCOV26 Observations EC14012-1446}
\tablehead{
\colhead{Run Name} & \colhead{Telescope} & \colhead{Detector} & \colhead{Date} & \colhead{Length} \\
\colhead{} & \colhead{(m)} & \colhead{} &\colhead{} & \colhead{(hrs)} 
}
\startdata
 hawa20080325-09& Hawaii 2.2  & E2V ccd47-10 & 2008-03-25 & 6.2 \\
 saao20080326-21& SAAO 1.0  & UCT CCD & 2008-03-26 & 5.9 \\
 tene20080327-20 & Tenerife 0.8  & TK1024 & 2008-03-27 & 3.0 \\
 saao20080327-20 & SAAO 1.0  & UCT CCD & 2008-03-27 & 7.5 \\
 saao20080328-20 & SAAO 1.0  & UCT CCD & 2008-03-28 & 7.3 \\
 saao20080329-20 & SAAO 1.0  & UCT CCD & 2008-03-29 & 7.2 \\
 tene20080330-03 & Tenerife 0.8  & TK1024 & 2008-03-30 & 2.9 \\
 saao20080330-20 & SAAO 1.0  & UTC CCD & 2008-03-30 & 7.5 \\
 saao20080331-20 & SAAO 1.0  & UTC CCD & 2008-03-31 & 7.1 \\
 mcdo20080401-05 & McDonald 2.1  & E2V ccd57-10 & 2008-04-01 &
 \phantom{1}6.1\tablenotemark{*} \\
 saao20080401-20 & SAAO 1.0  & UTC CCD & 2008-04-01 & 5.4 \\
 loia20080403-00 & Loia 1.52  & EEV 1300x1340B & 2008-04-03 & 1.1 \\
 ctio20080403-01 & CTIO 0.9  & $\rm{Tek2K_3}$ & 2008-04-03 & 7.5 \\
 soar20080403-02 & SOAR 4.1 & 2Kx4K MIT/Lincoln Lab CCD & 2008-04-03 &
 \phantom{1}7.6\tablenotemark{*} \\
 sara20080403-05 & SARA 1.0  & CCD & 2008-04-03 & 6.3 \\
 mcdo20080403-08 & McDonald 2.1  & E2V ccd57-10 & 2008-04-03 & 3.0 \\
 saao20080403-20 & SAAO 1.0  & UCT CCD & 2008-04-03 & 6.8 \\
 salt20080403-21 & SALT 10.0 & CCD & 2008-04-03 & 1.0 \\
 soar20080404-01 & SOAR 4.1 & CCD & 2008-04-04 & \phantom{1}7.7\tablenotemark{*}\\
 salt20080404-02 & SALT 10.0 & E2V 44-82  & 2008-04-04 & 0.7 \\
 ctio20080404-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-04 & 7.0 \\
 mcdo20080404-05 & McDonald 2.1 & E2V ccd57-10 & 2008-04-04 &
 \phantom{1}5.4\tablenotemark{*} \\
 sara20080404-10 & SARA 1.0 & CCD & 2008-04-04 & 0.6 \\
 saao20080404-21 & SAAO 1.0 & UTC CCD & 2008-04-04 & 6.4 \\
 salt20080404-21 & SALT 10.0 & E2V 44-82 &2008-04-04 & 1.0 \\
 soar20080405-01 & SOAR 4.1 & 2Kx4K MIT/Lincoln Lab CCD & 2008-04-05 &  \phantom{1}4.7\tablenotemark{*} \\
 salt20080405-02 & SALT 10.0 & E2V 44-82 & 2008-04-05 & 1.0 \\
 ctio20080405-03 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-05 & 6.3 \\
 mcdo20080405-09 & McDonald 2.1 & E2V ccd57-10 & 2008-04-05 & 1.7 \\
 mtjo20080405-11 & Mt. John 1.0 & E2V ccd57-10 & 2008-04-05 & 3.3 \\
 boao20080405-14 & BOAO 1.8 & SITe SI424AB CCD & 2008-04-05 & 4.4 \\
 salt20080405-21 & SALT 10.0 & E2V 44-82& 2008-04-05 & 1.0 \\
 saao20080405-22 & SAAO 1.0 & UTC CCD & 2008-04-05 & 3.1 \\
 salt20080406-01 & SALT 10.0 & E2V 44-82 & 2008-04-06 & 1.0 \\
 soar20080406-02 & SOAR 4.1 &2Kx4K MIT/Lincoln Lab CCD & 2008-04-06 &
 \phantom{1}7.3\tablenotemark{*} \\
 mcdo20080406-09 & McDonald 2.1 & E2V ccd57-10 & 2008-04-06 & 2.0 \\ 
 ctio20080407-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-06 & 6.2 \\
 mcdo20080407-08 & McDonald 2.1 & E2V ccd57-10 & 2008-04-07 & 3.1 \\
 boao20080407-15 & BOAO 1.8 & SITe SI424AB CCD & 2008-04-07 & 4.0 \\
 saao20080407-20 & SAAO 1.0 & UTC CCD & 2008-04-07 & 5.9 \\
 salt20080407-20 & SALT 10.0 & E2V 44-82 & 2008-04-07 & 1.0 \\
 salt20080408-01 & SALT 10.0 & E2V 44-82 & 2008-04-08 & 1.0 \\
%\tablebreak
 ctio20080408-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-08 & 1.8 \\
 mcdo20080408-09 & McDonald 2.1 & E2V ccd57-10 & 2008-04-08 & 1.5 \\
 luli20080408-14 & Lulin 1.0 & E2V CCD36-40 & 2008-04-08 & 2.6 \\
 saao20080408-20 & SAAO 1.0 & UTC CCD & 2008-04-08 & 4.9 \\
 ctio20080409-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-09 & 6.6 \\
 mcdo20080409-09 & McDonald 2.1 & E2V ccd57-10 & 2008-04-09 & 0.6 \\
 ctio20080410-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-10 & 6.9 \\
 boao20080410-14 & BOAO 1.8 & SITe SI424AB CCD & 2008-04-10 & 3.0 \\
 ctio20080411-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-11 & 6.6 \\
 mcdo20080411-09 & McDonald 2.1 & E2V ccd57-10 & 2008-04-11 & 1.5 \\
 mcdo20080412-06 & McDonald 2.1 & E2V ccd57-10 & 2008-04-12 & 0.3 \\
 kpno20080412-07 & KPNO 2.0 & E2V ccd47-10 & 2008-04-12 & 3.7 \\
 ctio20080413-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-13 & 4.4 \\
 mcdo20080413-06 & McDonald 2.1 & E2V ccd57-10 & 2008-04-13 & 4.7 \\
 ctio20080414-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-14 & 7.1 \\
 kpno20080414-04 & KPNO 2.0 & E2V ccd47-10 & 2008-04-14 & 2.4 \\
 lash20080414-08 & Las Cumbres 2.0 &E2V CCD42-40  & 2008-04-14 & 3.4 \\
 mcdo20080414-09 & McDonald 2.1 & E2V ccd57-10 & 2008-04-14 & 1.7 \\
 luli20080414-17 & Lulin 1.0 & E2V CCD36-40 & 2008-04-14 & 2.4 \\
 ctio20080415-02 & CTIO 0.9 & $\rm{Tek2K_3}$ & 2008-04-15 & 6.6 \\
 lash20080415-09 & Las Cumbres 2.0 & E2V CCD42-40  & 2008-04-15 & 3.8 \\
 luli20080415-16 & Lulin 1.0 & E2V ccd36-40 & 2008-04-15 & 4.3 \\
 mabu20080415-20 & Mt. Abu 1.2 & TEK CCD & 2008-04-15 & 1.3 \\
 mabu20080416-20 & Mt. Abu 1.2 & TEK CCD & 2008-04-16 & 2.2 \\
 kpno20080417-09 & KPNO 2.0 & E2V ccd47-10  & 2008-04-17 & 2.8 \\
 kpno20080418-07 & KPNO 2.0 & E2V ccd47-10 & 2008-04-18 & 3.9 \\
 braz20080426-04 & LNA 1.6 & WI106 CCD & 2008-04-26 & 2.1 \\
 braz20080427-05 & LNA 1.6 & WI106 CCD & 2008-04-27 & 1.9 \\
 braz20080428-04 & LNA 1.6 & WI106 CCD & 2008-04-28 & 1.9 \\
 braz20080429-05 & LNA 1.6 & WI106 CCD & 2008-04-29 & 1.2 \\
\enddata
%\tablenotetext{}{All observations are CCD.}
\tablenotetext{*}{High signal to noise light curves used for light curve fitting. All other observations were used to obtain accurate frequency information.}

\label{tab:journal}
\end{deluxetable}


==> provencaltab4.tex <==
\begin{deluxetable}{rrrrr} 
%\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Frequency ($l,m$) Identifications}
\tablewidth{0pt}
\tablehead{
\colhead{Frequency} & \colhead{Period} & \colhead{Combination} & \colhead{Asteroseismology} &\colhead{Final Nonlinear Fit}  \\
\colhead{\muHz} & \colhead{(s)} & \colhead{($l,m$)}
&\colhead{($l,m$)} & \colhead{($l,m$)}}
\startdata
$935.3799\pm0.002$ & 1069.085 &  &(1,any) & (2,-1)\\
$1021.139\pm0.002$ & 979.299 & &(1,any) & (2,2)\\
$1104.252\pm0.001$ & 905.591 &  &(1,any) & (2,1)\\
$1155.925\pm0.002$ & 865.108 &  &(1,any) & (2,2)\\
$1241.403\pm0.002$ & 805.540 &  & (1,any)& (2,2) \\
$1418.369\pm0.002$ & 705.035 &  &(2,any)  & (2,1)\\
$1521.575\pm0.002$ & 657.214 &  & (1,1) & 1,1)\\
$1548.146\pm0.001$ & 645.933 & (1,0) & (1,any) & (1,0)\\
$1624.015\pm0.003$ & 615.758 & (1,1) & (1 1) & (1,1)\\
$1633.907\pm0.001$ & 612.030 & (1,0) & (1,0/1) & (1,1)\\
$1774.989\pm0.100$ & 563.384 & (1,-1) & (1,any) & (1,1)\\
$1860.248\pm0.400$ & 537.563 & &(2,any)  & (2,0)\\
$1883.555\pm0.003$ & 530.911 &  & (1,1)& (1,1)\\
$1887.404\pm0.001$ & 529.828 & (1,0) & (1,0)  & (1,0)\\
$1891.142\pm0.002$ & 528.781 & (1,-1) & (1,-1) & (1,-1)\\
$2304.745\pm0.001$ & 433.887 & (1,-1) & (2,any)  & (1,0)\\
$2504.897\pm0.001$ & 399.218 & (1,1) & (1,1) & (1,0) \\
$2508.060\pm0.002$ & 398.715 & (1/2,1/0) & (1,0) & (1,-1)\\
$2856.155\pm0.002$ & 350.121 & (2,0/1)& (2,any) & (2,0)
\enddata
\label{tab:freqid}
%% Text for table notes should follow after the \enddata but before
%% the \end{deluxetable}. Make sure there is at least one \tablenotemark
%% in the table for each \tablenotetext.
%\tablecomments{Table \ref{journal} is published in its entirety in the
%electronic edition of the {\it Astrophysical Journal}.  A portion is
%shown here for guidance regarding its form and content.}
%\tablenotetext{a}{Sample footnote for table~\ref{journal} that was generated
%with the deluxetable environment}
%\tablenotetext{b}{Another sample footnote for table~\ref{journal}}
\end{deluxetable}




==> provencaltab6.tex <==
\begin{deluxetable}{rrrrrrrr} 
%\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Stellar Parameters}
%\tablewidth{0pt}
\tablehead{
\colhead{Star} & \colhead{\teff(K)} & \colhead{log g} &
\colhead{Period (s)} & \colhead{$\tau_0$(s)} &\colhead{$\rm{P_{max}}$}& \colhead{$\theta$} &
\colhead {$N$} \\
%\colhead{} & \colhead{(K)} & \colhead{} &\colhead{s} &\colhead{s} & \colhead{} & \colhead{}\\ 
}
\startdata
G117-B15A & $12010\pm180$ & 8.33 & 215.2 &$30\pm\phantom{1}10$ &
$188\pm\phantom{10}63$ & --- & ---\\
EC14012-1446 & $11768\pm\phantom{1}23$ & 8.11 & 612.3 &
$99\pm\phantom{1}12$ &
$624\pm\phantom{10} 75$ &$33\pm\phantom{1}3$ & $85\pm\phantom{1}6$  \\
G29-38 & $11690\pm120$ & 8.11 & 615.2& $187\pm\phantom{1}20$ &
$1177\pm\phantom{1}126$
&$66\pm\phantom{1}3$ & $95\pm\phantom{1}8$  \\
WDJ1524-0030 & $11660\pm180$ & 8.06 & 697.3 & $163\pm\phantom{1}35$
&$1024\pm\phantom{1}220$ &$58\pm10$ & $95\pm15$  \\
GD154 & $11270\pm170$ & 7.95& 1185.9 & $1169\pm200$ & $7345\pm1257$ &
$10\pm10$ & $127\pm25$ 
\enddata
\label{tab:stars}
%% Text for table notes should follow after the \enddata but before
%% the \end{deluxetable}. Make sure there is at least one \tablenotemark
%% in the table for each \tablenotetext.
\tablecomments{\teff\ measurements are from \citet{Koester09},
  \citet{KH01}, \citet{Koester00}.  Given pulsation periods are for
  the largest amplitude frequency. Entries marked with ``---'' did not
  have unique values determined by the fits.  }

%electronic edition of the {\it Astrophysical Journal}.  A portion is
%shown here for guidance regarding its form and content.}
%\tablenotetext{a}{Sample footnote for table~\ref{tbl-1} that was generated
%%\tablenotetext{b}{Another sample footnote for table~\ref{tbl-1}}
\end{deluxetable}



